Lodos-v2: An Efficient Primal Formulation of the Exact Frictional Contact Problem

Lodos-v2 is a GPU-based simulation framework for massively parallel rigid-body dynamics with contact. It is specifically designed to achieve high throughput in scenes involving collisions among large numbers of detailed meshes. Its predecessor, Lodos-v1, had two main limitations. First, it solved the standard convex relaxation of cone-complementarity-based contact dynamics, thereby inheriting well-known physical artifacts, including lift-off and artificial compliance in the normal direction, as well as creep in the tangential direction. Second, its contact-group reparameterization scheme, which rescales spring-damper forces using a single factor per collision pair, could not be integrated with other constraints required by a full-fledged simulator, such as joint limits and welds. Lodos-v2 addresses both limitations through two main contributions. First, it introduces an efficient algorithm for solving the exact frictional contact problem by sequentially solving a cascade of convex relaxations in primal form within an outer proximal minimization loop. Second, it extends the contact-group reparameterization scheme of Lodos-v1 to the primal formulation of cone-complementarity-based contact dynamics, enabling its integration with the other constraints of a full-fledged simulator. Experiments demonstrate that these contributions result in throughput improvements over established rigid-body simulation frameworks. The source code is available at https://github.com/martius-lab/lodos.

==> contact_notation.tex <==
\RequirePackage{mathtools,amssymb,bm}

\newcommand{\vct}[1]{\bm{#1}}
\newcommand{\gvec}[1]{\mathbf{#1}}
\newcommand{\mat}[1]{\mathbf{#1}}
\newcommand{\cset}[1]{\mathcal{#1}}
\newcommand{\reals}{\mathbb{R}}
\providecommand{\trsp}{\mathsf{T}} %

\newcommand{\vx}{\vct{x}}
\newcommand{\vy}{\vct{y}}
\newcommand{\vz}{\vct{z}}
\newcommand{\vs}{\vct{s}}
\newcommand{\vw}{\vct{w}}
\newcommand{\vp}{\vct{p}}
\newcommand{\vn}{\vct{n}}
\newcommand{\vt}{\vct{t}}
\newcommand{\vg}{\vct{g}}
\newcommand{\va}{\vct{a}}
\newcommand{\vb}{\vct{b}}
\newcommand{\vd}{\vct{d}}
\newcommand{\ve}{\vct{e}}
\newcommand{\vf}{\vct{f}}
\newcommand{\vh}{\vct{h}}
\newcommand{\vu}{\vct{u}}
\renewcommand{\vv}{\vct{v}}
\newcommand{\vlambda}{\vct{\lambda}}
\newcommand{\vmu}{\vct{\mu}}
\newcommand{\vsigma}{\vct{\sigma}}
\newcommand{\vtau}{\vct{\tau}}
\newcommand{\vgamma}{\vct{\gamma}}
\newcommand{\zerovec}{\vct{0}}
\newcommand{\onesvec}{\vct{1}}
\newcommand{\identity}{\mat{I}}
\newcommand{\mA}{\mat{A}}

\newcommand{\gpos}{\gvec{q}}
\newcommand{\gvel}{\gvec{v}}
\newcommand{\gacc}{\gvec{a}}
\newcommand{\gbias}{\gvec{b}}
\newcommand{\forces}{\gvec{f}}
\newcommand{\dualrhs}{\gvec{r}}
\renewcommand{\freeacc}{\gacc_f}
\newcommand{\freevel}{\gvel_f}
\newcommand{\contactvels}{\bar{\vv}}
\newcommand{\freecontactvels}{\contactvels_f}
\newcommand{\contactjac}{\bar{\jacmat}}
\newcommand{\refacc}[1]{\va_{\mathrm{ref},#1}}
\newcommand{\refaccs}{\bar{\va}_{\mathrm{ref}}}
\newcommand{\stacked}[1]{\bar{#1}}
\newcommand{\massmat}{\mat{M}}
\newcommand{\bodymassmat}{\mat{M}}
\newcommand{\coriolismat}{\mat{C}}
\newcommand{\delassus}{\mat{G}}
\newcommand{\regularizer}{\mat{R}}
\newcommand{\regentry}{R} %
\newcommand{\rotmat}{\mat{R}}
\newcommand{\inertiatensor}{\mat{I}}
\newcommand{\kinmap}{\mat{N}}
\newcommand{\frictionbasis}{\mat{B}}
\newcommand{\correction}{\vct{\Gamma}}
\newcommand{\timestep}{\Delta t}
\newcommand{\timehorizon}{T}
\newcommand{\frictioncoef}{\mu}
\newcommand{\stabilization}{\gamma}
\newcommand{\signedgap}{d}
\newcommand{\nq}{n_q}
\newcommand{\nv}{n_v}
\newcommand{\ncontacts}{N}
\newcommand{\nfrictiondirs}{K}

\newcommand{\SOthree}{\ensuremath{\mathrm{SO}(3)}}
\newcommand{\SEthree}{\ensuremath{\mathrm{SE}(3)}}
\newcommand{\sothree}{\ensuremath{\mathfrak{so}(3)}}
\newcommand{\sethree}{\ensuremath{\mathfrak{se}(3)}}
\newcommand{\unitsphere}{\mathbb{S}^{2}}
\newcommand{\ddt}{\frac{\mathrm{d}}{\mathrm{d}t}}
\newcommand{\crossmat}[1]{\left[#1\right]}

\newcommand{\convset}{\cset{C}}
\newcommand{\complset}{\cset{S}} %
\newcommand{\cone}{\cset{K}}
\newcommand{\frictioncone}[1]{\cone_{#1}}
\newcommand{\dualcone}[1]{{#1}^{*}}
\newcommand{\polarcone}[1]{{#1}^{\circ}}

\newcommand{\projop}{\operatorname{P}}
\newcommand{\proj}[1]{\projop_{#1}}
\newcommand{\normalcone}[1]{\operatorname{N}_{#1}}
\newcommand{\normalbasis}[1]{\mat{N}_{#1}}
\newcommand{\jacmat}{\mat{J}}
\newcommand{\jac}[1]{\jacmat_{#1}}
\newcommand{\projjac}[1]{\jac{\proj{#1}}}
\DeclareMathOperator{\linspan}{span}
\DeclareMathOperator{\colspace}{colspace}
\DeclareMathOperator{\concat}{concat}
\DeclareMathOperator{\diagop}{diag}
\DeclareMathOperator{\ncpop}{NCP}
\providecommand{\argmin}{\operatorname*{arg\,min}}
\providecommand{\argmax}{\operatorname*{arg\,max}}

\DeclarePairedDelimiter{\norm}{\lVert}{\rVert}
\DeclarePairedDelimiter{\abs}{\lvert}{\rvert}
\DeclarePairedDelimiterX{\inner}[2]{\langle}{\rangle}{#1,\,#2}
\DeclarePairedDelimiterX{\setof}[2]{\lbrace}{\rbrace}{%
  #1\,\delimsize\vert\,#2}

